Quantile Multi-Armed Bandits: Optimal Best-Arm Identification and a Differentially Private Scheme

We study the best-arm identification problem in multi-armed bandits with stochastic, potentially private rewards, when the goal is to identify the arm with the highest quantile at a fixed, prescribed level. First, we propose a (non-private) successive elimination algorithm for strictly optimal best-arm identification, we show that our algorithm is $\delta$-PAC and we characterize its sample complexity. Further, we provide a lower bound on the expected number of pulls, showing that the proposed algorithm is essentially optimal up to logarithmic factors. Both upper and lower complexity bounds depend on a special definition of the associated suboptimality gap, designed in particular for the quantile bandit problem, as we show when the gap approaches zero, best-arm identification is impossible. Second, motivated by applications where the rewards are private, we provide a differentially private successive elimination algorithm whose sample complexity is finite even for distributions with infinite support-size, and we characterize its sample complexity. Our algorithms do not require prior knowledge of either the suboptimality gap or other statistical information related to the bandit problem at hand.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%parenthesis
\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}

% typeface macros
\newcommand{\mbf}{\mathbf}
\newcommand{\mc}{\mathcal}
\newcommand{\mrm}{\mathrm}
\newcommand{\msf}{\mathsf}
\newcommand{\tb}{\textbf}
\newcommand{\mbb}{\mathbb}
\newcommand{\bds}{\boldsymbol}
% editing macros
\usepackage[dvipsnames]{xcolor}
\usepackage[normalem]{ulem}
\newcommand{\cn}{\textcolor{red}{[\raisebox{-0.2ex}{\tiny\shortstack{citation\\[-1ex]needed}}]}}
\newcommand{\ads}[1]{\textcolor{magenta}{\textbf{ADS:} #1}}
\newcommand{\kn}[1]{\textcolor{red}{\textbf{KN:} #1}}
\newcommand{\dk}[1]{\textcolor{red}{\textbf{DK:} #1}}
\newcommand{\os}[1]{\textcolor{red}{\textbf{OS: #1}}}
\newcommand\redout{\bgroup\markoverwith{\textcolor{red}{\rule[.5ex]{2pt}{0.4pt}}}\ULon}
\newcommand{\edit}[2]{\redout{#1}{~\textcolor{blue}{#2}}}
\newcommand{\todo}[1]{\textcolor{red}{\textbf{TODO:} #1}}

\renewcommand{\P}{\mbb{P}}
\newcommand{\E}{\mbb{E}}
\newcommand{\Var}{\mathop{\mathrm{Var}}\nolimits}
\newcommand{\var}{\text{VaR}_{1-\alpha}}
\newcommand{\uaX}{u_{\alpha}(X)}
\newcommand{\euaX}{\hat{u}_{\alpha}(X)}
%\DeclareMathOperator\arctanh{arctanh}
%\DeclareMathOperator\Pre{Pre}
\newcommand*{\QEDA}{\null\nobreak\hfill\ensuremath{\blacksquare}}%
\newcommand*{\QEDB}{\null\nobreak\hfill\ensuremath{\square}}
% distributions
\newcommand{\ind}[1]{\mbf{1}_{#1}}
\newcommand{\bern}{\mathrm{Bernoulli}}
\newcommand{\Rad}{\mathrm{Rademacher}}
\newcommand\defeq{\stackrel{\triangle}{=}}
\newcommand{\SKL}{\bds{S}_{\text{KL}}}
\newcommand{\KL}[2]{\bds{D}_{\text{KL}}( #1 \| #2 )}

\newcommand{\tpath}{\mathrm{path}}

\newcommand{\ssTV}{\mathrm{ssTV}}

\newcommand{\dtv}{d_{\mathrm{TV}}}
\newcommand{\dflip}{d_{\mathrm{flip}}}

%% Define macros for notation noiseless vs noisy setting%
\newcommand{\bx}{\mbf{x}}
\newcommand{\bX}{\mbf{X}}
\newcommand{\bnX}{\mbf{Y}} %noisy X
\newcommand{\bnx}{\mbf{y}}
\newcommand{\nX}{Y} %noisy X
\newcommand{\nx}{y}
\newcommand{\nmu}{\mu^{\dagger}} % noisy \mu
\newcommand{\nmue}{\hat{\mu}^{\dagger}} %estimate of noisy \mu
\newcommand{\np}{\p_{\dagger}}
%%%\T and \p are changed in theorems and lemmas
\newcommand{\T}{\mathrm{T}}%original tree
\newcommand{\p}{\mathrm{p}}% pmf
\newcommand{\TCL}{\T^\mathrm{CL}}%CL tree
\newcommand{\TCLn}{\T^\text{CL}_{\dagger}}%CL tree noisy setting
\newcommand{\N}{N} %noise RV
\newcommand{\n}{n}%number of samples
\newcommand{\nn}{n_{\dagger}}%number of samples noisy
\newcommand{\neps}{\epsilon_{\dagger}}
\newcommand{\eps}{\epsilon}
\newcommand{\neta}{\eta^{\dagger}}
\newcommand{\ngam}{\gamma_{\dagger}}
\newcommand{\ntau}{\tau^{\dagger}}
%\newcommand{\nP}{P^{\dagger}}
\newcommand{\nPe}{\hat{P}^{\dagger}}
\newcommand{\nZ}{Z_{\dagger}}
\newcommand{\Lnorm}{\mc{L}^{(2)}}
\newcommand{\RIP}{\Pi{}_{\TCL}} 
\newcommand{\RIPn}{\Pi{}_{\TCLn}}
\newcommand{\treedistr}{\mc{P}_{\T}(c_1,c_2)}
\newcommand{\isingforest}{\mc{P}_{\T}(0,\beta)}
\newcommand{\er}{\hat{\rho}}
\newcommand{\CP}{\mc{CP}_{\T}}
\newcommand{\Vast}{\bBigg@{5}}

%%% Macros for the 6 events%%%%%%%
%\newcommand{\Err}{\mathrm{E}}
%\newcommand{\Ecorr}{\mathrm{E}^{\text{corr}}\left(\epsilon\right)}
%\newcommand{\Ecasc}{\mathrm{E}^{\text{cascade}}\left(\gamma\right)}
%\newcommand{\Estrong}{\mathrm{E}^{\text{strong}}\left(\epsilon\right)}
%\newcommand{\Ecorrn}{\mathrm{E}_{\dagger}^{\text{corr}}\left(\neps\right)}
%\newcommand{\Ecascn}{\mathrm{E}_{\dagger}^{\text{cascade}}\left(\ngam\right)}
%\newcommand{\Estrongn}{\mathrm{E}_{\dagger}^{\text{strong}}\left(\neps\right)}
%\newcommand{\Eedge}{\mathrm{E}_{e}^{\text{edge}}}
%\newcommand{\EedgeA}{\mathrm{E}^{\text{edge}}(\mc{A})}
%\newcommand{\EedgeAd}{\mathrm{E}^{\text{edge}}(\mc{A}_d)}
%\newcommand{\EedgeET}{\mathrm{E}^{\text{edge}}(\mc{E}_{\T})}
%\newcommand{\BSC}{\mathrm{BSC}(q)^p}
%%%%%%%% Extra notation --- Proofs' Section %%%%%%%%%%

%%%%%% Variable for the noise%%%%%%%% 
%\newcommand{\Nw}{N_{w}}
%\newcommand{\Nwb}{N_{\bar{w}}}
%\newcommand{\Nu}{N_{u}}
%\newcommand{\Nub}{N_{\bar{u}}}
%\newcommand{\Zsample}{Z_{e,u,\bar{u}}^{(i)}}
%\newcommand{\Z}{Z_{e,u,\bar{u}}}
%\newcommand{\Ysample}{M_{e,u,\bar{u}}^{(i)}}
%\newcommand{\Y}{M_{e,u,\bar{u}}}
%\newcommand{\Zf}{Z_{f,u,\bar{u}}}
%\newcommand{\Zfsample}{Z_{f,u,\bar{u}}^{(i)}}
%\newcommand{\Yf}{M_{f,u,\bar{u}}}
%\newcommand{\Yfsample}{M_{f,u,\bar{u}}^{(i)}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\DKL}{D_{\text{KL}}}


%\newcommand{\Ith}{\mathbf{I}^{\mathrm{thres}}}
%\newcommand{\Ith}{\mathbf{I}^o}
%\newcommand{\MI}{\hat{I}}
%\newcommand{\fset}{\mc{E}\mc{V}^2}


\DeclareMathOperator{\gap}{gap}
\newcommand{\gapx}{\gap(x)}
\newcommand{\epochgap}{\Gamma_e}
\renewcommand{\Pr}{\P}
